On the Efficiency of K-Means Clustering: Evaluation, Optimization, and Algorithm Selection

This paper presents a thorough evaluation of the existing methods that accelerate Lloyd's algorithm for fast k-means clustering. To do so, we analyze the pruning mechanisms of existing methods, and summarize their common pipeline into a unified evaluation framework UniK. UniK embraces a class of well-known methods and enables a fine-grained performance breakdown. Within UniK, we thoroughly evaluate the pros and cons of existing methods using multiple performance metrics on a number of datasets. Furthermore, we derive an optimized algorithm over UniK, which effectively hybridizes multiple existing methods for more aggressive pruning. To take this further, we investigate whether the most efficient method for a given clustering task can be automatically selected by machine learning, to benefit practitioners and researchers.

==> graph/analysis.tex <==
\shengnew{\section{Complexity Analysis and Comparison}
The complexity of time and space will be analysis.
Probality of being pruned.
Data access, bound access, bound computing, distance computing will compose the model.
As shown in Table~\ref{tab:com}, we compare the complexity.

\subsection{Baseline}
nkt distance computations.

data access, when k centroids are in the cache, we will further increase the performance. \cite{Bender2015}

We have a bound of visited nodes, upper bound and lower bound.

Why we need an evaluation, as we observe that no algorithm can be the best all the time for all the datasets. 
We evaluate all the algorithms by considering all the factors, and propose a unified algorithm.

Existing algorithm scikit-learn use ``Elkan’s algorithm" which published in 2003, \cite{scikit}.

In practice, the k-means algorithm is very fast (one of the fastest clustering algorithms available), but it falls in local minima. That’s why it can be useful to restart it several times. 

Estimating the number of clusters also needs multiple running.

Space cost.

We use histogram to visualize the main cost as shown in the Table.
The bound space is big.



}

\iffalse
\section{Complexity Analysis}
\label{sec:complex}

As clustering efficiency is highly sensitive to the dataset \cite{Kanungo2002}, we will have an analysis on the time and complexities as below:

\subsection{Computing Model}
Distance computation: $l$-norm $\mathcal{O}(d)$.

Bound computation: $\mathcal{O}(1)$.

Data and bound access.

The overall time is composed by:

1) the index constructing time ($\mathcal{O}(nlogn)$;

2) index traversing time, including building the Voronoi diagram between $k$ centroids in the beginning ($\mathcal{O}(klogk+k^{\lceil \frac{d}{2}\rceil})$ \cite{Chazelle1993}). For every node, it needs to find the nearest centroid first which cost $O(kd)$; then the time pruning time using in judging whether the node in kd-tree intersects with the $k-1$ hyperplane, 

While our method is much $O(kd+k)$ at most, and we can further use bound to prune large proportion of them.

3) the point assignment time, the percentage of pruning of distance computation.

And the apportioned cost on each iteration as we only need a single traversal over the tree.

\subsection{Worst Case Study}
The worst case, 
when all the nodes cannot be pruned, we show the cost of index-based, ours, and sequential.

The complexity depends on the dimensionality $d$ and the possibility of node being pruned (related to the depth and number of points inside, and the iteration $t$).

Reference paper on theory analysis: \cite{Kanungo2002,Blomer2016,GEORGOGIANNIS2016,Arthur2011}
\fi

==> graph/plot.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usepackage{csvsimple}
\usepackage{pgfplotstable}

\usepackage[markup=none,commentmarkup=footnote]{changes}
\usepackage{color}
\definechangesauthor[color=magenta]{AE}
%%% Alternative definition to have the remarks
%%% in the margins instead of footnotes
%% Crude definition of a plain remark/note using \added from changes
%\newcommand{\note}[2][]{\added[id=#1,comment={\color{authorcolor}#2}]{}}


\DeclareMathOperator{\sign}{sgn}

\definecolor{blue}{RGB}{8,141,165}
\definecolor{olivegreen}{RGB}{85,107,47}
\definecolor{orange}{RGB}{229,148,0}
\definecolor{marine}{RGB}{0,32,96}
\definecolor{maroon}{RGB}{178, 50, 50}


\pgfplotsset{every tick label/.append style={font=\tiny}}
\pgfplotsset{
	box plot width/.initial=4em,
	box plot/.style={
		/pgfplots/.cd,
		black,
		only marks,
		mark=-,
		mark size=\pgfkeysvalueof{/pgfplots/box plot width},
		/pgfplots/error bars/.cd,
		y dir=plus,
		y explicit,
	},
	box plot box/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\draw [line width=0.20mm]  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
		},
		/pgfplots/table/.cd,
		y index=2,
		y error expr={\thisrowno{3}-\thisrowno{2}},
		/pgfplots/box plot
	},
	box plot top whisker/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark}%
			{\pgfplotserrorbarsmark}%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
			{\pgfplotserrorbarsmarkopts}%
			\path ##1 -- ##2;
		},
		/pgfplots/table/.cd,
		y index=4,
		y error expr={\thisrowno{2}-\thisrowno{4}},
		/pgfplots/box plot
	},
	box plot bottom whisker/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark}%
			{\pgfplotserrorbarsmark}%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
			{\pgfplotserrorbarsmarkopts}%
			\path ##1 -- ##2;
		},
		/pgfplots/table/.cd,
		y index=5,
		y error expr={\thisrowno{3}-\thisrowno{5}},
		/pgfplots/box plot
	},
	box plot median/.style={
		/pgfplots/box plot
	}
}
\pgfplotsset{yticklabel style={text width=1.0em,align=right}}
\pgfplotsset{compat=1.12}

\pgfplotstableread[col sep = comma]{graph/CLKeasy_results.csv}\CLKeasy


==> related.tex <==
\section{Related Work}
Selecting algorithms or configurations to achieve high performance have been investigated in meta-learning for effectiveness and database tuning for efficiency, respectively.
%Traditional method let experienced analysts to configure in a manual way, which is also known as rule-based which are DBAs' experience.
%subsection{Configuration Tuning}

\myparagraph{Algorithm Selection and Configuration}
%\cite{Munoz2018}
The task of algorithm selection involves choosing an algorithm from a set of algorithms in order to exploit the varying performance of algorithms over a set of instances \cite{Bischl2016}.
Generally, learning to configure algorithms \cite{Bengio2020} augment an operation research algorithm with valuable pieces of information.
This is also known as the automatic design of solutions (workflows/pipeline), which is a promising direction that needs more effort.
The automatic design of complete pipelines of algorithms to solve problems has inspired several open-source prototypes, such as auto-weka \cite{Thornton2012} and auto-sklearn \cite{Feurer2015}.

For \kmeans clustering algorithm selection, Balcana et al. \cite{Balcana} proposed to learn a parameter for controlling the initialization procedure, and another parameter controlling the local search procedure, to solve the problem of random initialization.
Balcana et al. \cite{Balcan2019} further learned to select the algorithm and distance metric to achieve a better local optimal, e.g., a smaller objective value.
However, the work related to clustering algorithm selection is to select the best algorithm with high effectiveness, but not efficiency which we focus on in this paper.
%We are the first to put the efficiency as the first target for clustering algorithm selection.
%Moreover, the main difference with our work is that meta-feature needs ground truth, i.e., it is supervised.

%\cite{Brazdil2018}
\iffalse
\subsection{Running time prediction}
By predicting the cost, DBAs can try multiple solutions and then choose the optimal configuration.
\cite{Wu2013a} predicted the query time for dynamic workload.
Instead of predicting the running time, we predict the configuration directly, which a more common way.
%\subsection{Rule-based tuning}

\subsection{Program auto-tuning}
Polyalgorithm is a set of algorithms together with rules for choosing when to use each one, how to determine the optimal rule configuration has been a vital direction.
\cite{Ansel2009}
\cite{Ansel2014}
\cite{Ding2015b} proposed autotuning algorithmic Choice for Input Sensitivity.
\cite{Ashouri2018} review the techniques for autotuning the optimal configuration.
\cite{Chen2018c}

\subsection{Parameter tuning}
Tuning the best parameter is a common technique in machine learning and distributed computing.
However, our focus on configuration is to predict whether to use index or a bound, so we do not need to conduct parameter tuning.
\citet{Duan2009} proposed to tune the parameters.
\fi

\myparagraph{Database Knob Tuning}
By running multiple rounds of experiments with various parameter and knob settings in database management systems (DBMS), 
machine learning can learn from the tuning logs and train a model, and further recommend a configuration automatically.
%Compared with rule-based model, it can further explore deep dependency among multiple knobs that cannot be covered by the rules.
Dana et al. \cite{VanAken2017} firstly presented an automated approach
that leverages past experience from DBAs and collects new information to tune DBMS configuration.
Li et al. \cite{Li2018g} applied deep reinforcement learning (DRL) to turn for query-aware database systems.
Zhang et al. \cite{Zhang2019b} designed an end-to-end automatic cloud database tuning system using DRL.
%Workload classification \cite{Zhang2019b,Li2018g}, self tuning of the knob configurations to achieve best performance for new query plans.

%\subsection{Difference with existing models}
%As an automatic configuration tuning for fast \kmeans clustering, 
The basic differences between \utune and database tuning are three-fold.
Firstly, the database tuning highly depends on DBAs' manual tuning experience, while \utune is unsupervised and does not need much human's efforts during evaluation and training.
%Firstly, we are the first work that autotunes configuration for a specific clustering algorithm instead of a database.
Secondly, the database tuning focuses more on system settings, e.g., the amount of memory to use for caches, while we focus on high-level algorithm part in a unified system setting.
%and existing models do not model the dataset but the query which we do not have, so existing tuning models cannot work here.
Thirdly, unlike database tuning for a given complex execution or query plan, we only input a parameter $k$ and is more data-oriented.

==> response.tex <==
\twocolumn[\centering{\huge\textbf{Response Letter to Reviewer Comments}}\vspace{5em}]
\setcounter{page}{1}
First of all, we would like to thank the meta-reviewer and reviewers for the constructive comments that have helped us to improve
our paper titled \emph{``On the Efficiency of {K}-Means Clustering: Evaluation, Optimization, and Algorithm Selection"}.
We have revised our paper accordingly and are re-submitting the
manuscript for further evaluation.
In this response letter, we outline how each concern from the meta-reviewer and reviewers was
addressed, and describe the changes that we have made to the paper.
To assist the assessment, we have highlighted in the revised manuscript all changes in {\textcolor{blue}{blue color}}, and have cross-referenced each change with a margin note in {\textcolor{Brown}{brown color}}. We have also highlighted several important statements with {\textcolor{Green}{green-colored underlines}}, indicating that these statements have been presented in the original manuscript and may have been overlooked in the first round of review. We have also fixed several small typos and improved the overall presentation. Thank you again for your time and efforts in reviewing our revised manuscript.


%We have also highlighted several important claims with {\textcolor{green}{green-colored underlines}} that have been presented in the original manuscript, in order to indicate that we have mentioned the importance of data distribution and \uni while they might be overlooked in the first round of review. We also fixed several small typos to improve the overall presentation. Thank you for your time and efforts reviewing our revised manuscript.

	
\section{Response to Meta Reviews}
\label{sec:meta}

\comments{Substantially more depth in the experiments including studying the effect of distribution of the clusters, dimensionality, and initial choice of starting points.}
\response{
%	The effect of distribution of clusters on the performance is hard to quantize as it is the distribution of results, and will not affect the clustering performance, and normally the data distribution will affect.
In the revised manuscript, we have considered all the three aspects in our experimental evaluations, and carefully discussed their effects. 

First, it is worth highlighting that we have already discussed about the effects of \textbf{data distributions} on the performance of clustering algorithms in our original manuscript. Specifically, in Section~\ref{sec:rskc}, we have extracted problem features related to data distribution such as the radius of index's leaf nodes for algorithm selection, and the results in Table~\ref{tab:precision} show that the performance of algorithms is correlated with those features related to data distributions. We highlighted the relevant text by green-colored underlines in the manuscript, and also quote them as below:
%In Section~\ref{sec:rskc} of our original manuscript, we have already pointed out the importance of data distribution, and proposed new features to indicate the distribution effect on algorithm selection. We highlight them by green-colored underlines for your reference, and quote them as below:

\vspace{0.2cm}	
\noindent\fbox{		\parbox{0.46\textwidth}{
		``\textit{{In addition to the basic features, we also extract novel and more complex features that can capture certain properties of data distribution based on our built index.} %Check more responses at \ref{sec:meta} and~\ref{sec:r2}.
			%By building index, we can get rich information about the data distribution, e.g., whether the data assemble well in the space.
			{Recall the pruning mechanisms in }Section~\ref{sec:frame}, {they work well when data shows good assembling distribution.} {The index construction actually conducts a more in-depth scanning of the data and reveals whether the data assemble well in the space.}
			{Specifically, the information we got includes the tree depth $h(T)$, number of leaf nodes $|N_l|$, number of internal nodes $|N_i|$, and imbalance of tree} {(i.e., the mean value and standard deviation of all leaf nodes' heights $h$)}.}''\\
		
		``\textit{Further, we extract more features of all the leaf nodes, including the radius of nodes $r$, the distance from child to parent nodes $\psi$, and the number of points in the leaf nodes $|L_p|$, during index construction.
			Specifically, we select all the leaf nodes $N$ and extract their $(r, \psi, |L_p|)$, then further compute their mean $\mu$ and standard deviation $\sigma$, which are all normalized by their maximum values in the tree.}''}} \\
		
Second, we have studied the effects of \textbf{dimensionality} on the indexing methods, and the results are presented in Figure~\ref{fig:index}. 
It shows that various indexing methods' performance will degrade with the increasing of dimensionality. %\yuan{What is summary of the results?} 
For sequential methods, we can also observe that the performance will degrade when testing the performance on high-dimensional datasets, such as BigCross and Covtype, as shown in Figure~\ref{fig:seq}. %\yuan{Where are the results?} 
To further investigate its effect on a specific dataset, we used the Mnist dataset to conduct experiments by increasing dimensionality $d$ ranging from 2, 10, 100, 200, 300, 400, 500, as shown in Figure~\ref{fig:increased}. 
%\yuan{What is the summary / key findings of Figure~\ref{fig:increased}?} 
We find that most algorithms can have a good performance in low dimension, and it is hard to maintain when tested with high-dimensional dataset. In contrast, \texttt{Drak}'s better performance in high-dimensional space also brings itself to the leader board in Figure~\ref{fig:lead}.
We also added it to the appendix of our supplementary file.

\begin{figure}[h]
	\vspace{-1em}
	\includegraphics[width=1\linewidth]{graph/NewPlotS/figure/increasingDimensions.eps}
		\vspace{-2.5em}
	\caption{The effect of increasing dimensionality on Mnist dataset.}
	\vspace{-1em}
	\label{fig:increased}
\end{figure}

Third, we have compared the effects of using two different \textbf{initialization} methods on the speedup, namely the random initialization and kmeans++ initialization \cite{Arthur2007}, respectively. The results are shown in Figure~\ref{fig:random1}. We can observe that the random initialization performs similarly to the kmeans++ initialization  when being tested with various algorithms and datasets. %Here, we fixed the total number of iterations to compare the pruning in a fair way, 
Since both initialization methods need various number of iterations to terminate, while kmeans++ usually needs fewer number of iterations and has been widely used (we also mentioned this in our original manuscript, see the green-colored underlines in Section~\ref{sec:accl}), we proceed to use the kmeans++ initialization for all the algorithms in the main paper, and do not present the detailed comparison in the main paper due to space limit.
%\yuan{I deleted ``the starting points will affect the clustering quality and the number of iterations...'', because it is not consistent with the experimental results.''}

%Second, the starting points will affect the clustering quality and the number of iterations. For example, random initialization by choosing $k$ points randomly has the problem of slow convergence, and existing work usually take the kmeans++ \cite{Arthur2007} as the default initialization method, as it needs few number of iterations to terminate. 
%In our experiments, we use the same group of initialized points; hence all the algorithms using one initialization method will need the same number of iterations and return the same results.
%We did not compare kmeans++ with the random initialization in our revised manuscript due to space limit, but we implemented both of them. After conducting experiments, the results reveal that the efficiency of same number of iterations is not affected much by two various initialization methods, as shown in Figure~\ref{fig:random1}, where the clustering speedups over Lloyd's algorithm are very similar in each dataset.


	
	
	%The data distributions did affect the algorithm's performance. To investigate how to select the proper algorithm according to the data distribution, we extracted relevant features such as the radius of index's leaf nodes. Table~\ref{tab:precision} shows that the radius has a relation with the performance of indexing and sequential solutions. This is because when the dataset assembles well, its index's leaf nodes will have a smaller radius, and it will be good for indexing methods to prune.
	
% 	For the dimensionality, we have shown its effect on the indexing method in Figure~\ref{fig:index}. For sequential methods, we can also observe that the performance will degrade when testing the performance on high-dimensional datasets, such as BigCross and Covtype.
% 	To further investigate its effect on a specific dataset, we used the Mnist dataset to conduct experiments by increasing dimensionality $d$ ranging from 2, 10, 100, 200, 300, 400, 500, as shown in Figure~\ref{fig:increased}. 
% 	We also added it to the appendix of our supplementary file.

	
%	\sheng{Experiments here on comparing two initializations, overall speedup.}
\begin{figure*}
	\centering
	\begin{minipage}{1\textwidth}
		\centering
		\hspace{-3.3em}\includegraphics[width=1.06\textwidth]{graph/legend.pdf}\\
		\hspace{-2.1em}\includegraphics[width=0.52\textwidth,height=0.11\textheight]{graph/NewPlotR/figure/all-dataset-speedup.eps}\hspace{-0.4em}
		\includegraphics[width=0.52\textwidth,height=0.11\textheight]{graph/NewPlotS/figure/all-dataset-speedup.eps}
		\vspace{-2em}
		\captionof{figure}{Overall speedup in various datasets when using random (left) and k-means++ initialization (right), respectively.}
		\vspace{-1.5em}
		\label{fig:random1}
	\end{minipage}\\
\end{figure*}
}


\comments{In addition, please explain in detail what is the rational and purpose of using UniK in this paper. Do we need it for the comparison? Does it work in the same way for all algorithms used in the paper or it may be creating unfair advantages for some algorithms?}
\response{The \textbf{primary purpose} of introducing \uni is to systematically review and compare existing algorithms that optimize the Lloyd's algorithm's efficiency in one system. The \uni framework concludes a common pipeline (see Figure~\ref{fig:workflow}) of most existing algorithms on how to prune unnecessary distance computations during assignments, and provides a clear taxonomy (two large groups: indexing and sequential) for these algorithms. With \uni, we can easily understand the similarities and differences between the existing algorithms. To our best knowledge, there has not been any framework that can cover so many algorithms like ours. Notably, we even included in our \uni a latest work that was just accepted to IEEE Transactions on Pattern Analysis and Machine Intelligence in July 2020,  during our revision.
	
	%In \uni, we first conclude a common pipeline (see Figure~\ref{fig:workflow}) of most existing algorithms on how to prune unnecessary distance computations during assignments. Readers can find a clear taxonomy (two large groups: indexing and sequential) and easily understand the focus of each algorithm and their major differences. 
	%\tocheck{To our best knowledge, there has not been any work that covered and reviewed so many algorithms in such a comprehensive way like our work, e.g., we even included a latest work just published at July 2020 during our revision.}
	
	%(and follow-up works in future)
	
	\textbf{We need \uni for the comparison}, because it enables a fine-grained performance breakdown of existing algorithms. This allows us to  evaluate existing algorithms more thoroughly using new metrics such as data accesses and bound updates (see Figures~\ref{fig:seq} to \ref{fig:seq2}). These measurements have never been used by any existing work, where the pruning ratio of distance computation was thought to be the only evaluation metric apart from the running time.
	
	\textbf{Our \uni does not create unfair advantages for any existing algorithm in comparison}, because an existing  algorithm corresponds to a certain knob configuration in \uni. In other words, by enabling certain knobs in \uni, we can recover an existing algorithm that runs in the same way as presented in the original paper. This will not incur any extra costs, so we do not create unfair advantages to any algorithm under comparison.
	%Note that we are the first to propose to evaluate not only based on pruning ratio.
	
	In addition, our \uni has the potential to provide an opportunity to further optimize existing algorithms to achieve a better performance. With the adaptive traversal configuration described in Algorithm~\ref{alg:kmeans} and Section~\ref{sec:travel}, \uni can become a new algorithm that combines the indexing and sequential methods to save more time during the assignment. Since this is the new optimization that has never been proposed, we think it is necessary to compare it with existing work, and we also verified its high performance in Section~\ref{sec:expuni} and Table~\ref{tab:overview}, respectively.
	
	%Finally, \uni paves the way to automatically predict the best algorithm for a given dataset, as our evaluation suggests that no single algorithm always performs the best on all datasets.
	
	We have highlighted the purpose and importance of \uni with green underlines in the introduction (Section~\ref{submission}) of the revised manuscript.}

% Finally, \uni is a framework that integrates multiple solutions and paves the way to automatically predict the optimal solutions for various datasets, as no optimal solutions exist for all tasks according to our evaluation. 
% To distinguish between existing algorithms and our proposed adaptive \uni algorithm, we call the auto-tuning method as \utune.

% Overall, our introduction (Section~\ref{submission}) has highlighted the above purpose and importance of \uni, especially the contribution part where we highlighted with green underlines.


\setcounter{cN}{1}
	
\section{Response to Reviewer \#1}
\label{sec:r1}
\comments{W2: The description of Section 5, i.e. the UniK framework, has some unclear points:\\
1) It is not clear to me how the existing methods are applied to the ``Node Assignment'' part in Section 5.1.1, specifically the Equation 9-11 (e.g. why Equation 11 holds). It could be better if that can be shown more explicitly.\\
2) The right part of Figure 4 is not clear to me, i.e. what happens to each cluster, why the centroid seems to be ``outside'' each cluster.\\
3) The knob problem described in W1.\\
4) In line 23, I could not find the meaning of $N_{rt}.v$, should it be vs instead?\\
5) In the last but one paragraph of Section 5, how the 2 adaptive traversal mechanisms are shown in Algorithm 1.}
\response{We have revised them one by one and hope that all concerns are resolved. Please check the corresponding places in the paper.\\
\textbf{1)}: We added references to Equation~\ref{equ:ball}, \ref{equ:notassign}, and Figure~\ref{fig:node}, which should be helpful to understand with an example.\\
\textbf{2)}: We moved the centroid into the cluster, and added a sentence to describe what will happen after it is inserted into the cluster.\\
\textbf{3)}: We added an example by turning on some knobs in the algorithm to run as a specific algorithm.\\
\textbf{4)}: Yes, it should be the sum vector $sv$.\\
\textbf{5)}: In the algorithm, we show a general case that we scan the nodes maintained in each cluster after the first iteration. 
Then both points and nodes in the cluster can be scanned using a unified framework, and the main difference is whether setting the radius $r$ as zero.
To be more adaptive, we can easily apply a strategy by inserting the root node again before each iteration, just like Line~\ref{line:aroot}. 
Due to space limit, we did not put it into the algorithm; instead, we used a paragraph to illustrate it as an alternative optimization.
}

\comments{W3: Some of the results showing in this paper are ``too detailed''.}
\response{For the histogram figures, we move the last three datasets that do not have much distinction to Appendix, such that the figures have better visibility. 
We put the full version of each figure across double columns, as shown in the appendix of our supplementary file.
	
	We also added more descriptions for the bold numbers. Here, we mainly want to show that both \uni and \utune can have much better results than the representative indexing and sequential algorithms, and \utune can be faster in most cases as it can predict the optimal bound configuration which performs better than a fixed configuration in \uni. 
}


\setcounter{cN}{0}
\section{Response to Reviewer \#2}
\label{sec:r2}
\comments{D1: The presentation can be further improved.}
\response{We have checked the whole paper and made much improvements.}

\comments{D2: It is good to set k from 10 to 1000 in all the experiments.}
\response{We have conducted new experiments by setting $k$ as 10, 100, 400, 700, and 1000, and the results are shown in Figure~\ref{fig:index}. We also show the results here in Figure~\ref{fig: index1} to facilitate your checking.
We can observe that Ball-tree, M-tree, and Cover-tree have very similar performance when $k\ge100$, and HKT and kd-tree's performances start to degrade.}
\begin{figure}
	\centering
	\includegraphics[width=9cm]{graph/legend-index.pdf}\\
	\includegraphics[width=0.4\linewidth]{graph/gnuplot/index-cluster-k.eps}
	\vspace{-1em}
	\caption{The effect of increasing $k$ on the performance of indexing methods.}
	\label{fig: index1}
	\vspace{-2.5em}
\end{figure}

\comments{D3: The auto-tuning method is very simple which depends on d, k and the dataset size.}
\response{
%\yuan{Do we need this response? Can we just say ``Please refer to the response to the meta-reviewer's Comment 1?}
In Section \ref{sec:rskc} of our original manuscript, we have highlighted that the data distribution is a key factor for the clustering algorithm selection (see green underlines), and it is not precise to use basic features for prediction. Here, we also paste our original claims as below:\\

\noindent\fbox{
	\parbox{0.46\textwidth}{
``\textit{{In addition to the basic features, we also extract novel and more complex features that can capture certain properties of data distribution based on our built index.} %Check more responses at \ref{sec:meta} and~\ref{sec:r2}.
%By building index, we can get rich information about the data distribution, e.g., whether the data assemble well in the space.
{Recall the pruning mechanisms in }Section~\ref{sec:frame}, {they work well when data shows good assembling distribution.} {The index construction actually conducts a more in-depth scanning of the data and reveals whether the data assemble well in the space.}
{Specifically, the information we got includes the tree depth $h(T)$, number of leaf nodes $|N_l|$, number of internal nodes $|N_i|$, and imbalance of tree} {(i.e., the mean value and standard deviation of all leaf nodes' heights $h$)}.}''\\


``\textit{Further, we extract more features of all the leaf nodes, including the radius of nodes $r$, the distance from child to parent nodes $\psi$, and the number of points in the leaf nodes $|L_p|$, during index construction.
	Specifically, we select all the leaf nodes $N$ and extract their $(r, \psi, |L_p|)$, then further compute their mean $\mu$ and standard deviation $\sigma$, which are all normalized by their maximum values in the tree.}''}}\\
%In this paper, we have extracted many features from datasets to describe the data distribution, and will extract more features in the future.

Then, we proposed to employ more advanced features, as shown in Table~\ref{tab:features}. In the table, we show not only the $k$, $d$, and $n$, but also multiple other features. Also, as shown in Table~\ref{tab:precision}, these advanced features will lead to much higher precision than $k$, $d$, and $n$ in the algorithm prediction, which proves that data distribution is an important feature for algorithm selection.}
%we have taken the data distribution into account.}


\comments{D4: As observed from Table 6, the improvement of auto-tuning is very small w.r.t. Unik for larger k values (i.e., 100 and 1000). Please clarify the reasons.}
\response{The goal of \utune is to select the fastest algorithm from the existing algorithms and our optimised \uni algorithm for a given clustering task. Therefore, \utune will not outperform the best algorithm in the selection pool on a given task. Since \uni performs well (likely to be the best performing algorithm in the selection pool) on most of the datasets when $k$ is large, it is reasonable that the improvement of \utune over \uni is small.
%and it does not mean that it has to be much faster than \uni. For example, if \uni is the fastest when $k$ is large, then \utune will return the same performance with \uni as \utune predicts the optimal algorithm as \uni, and run as the same configuration with \uni.
}

\comments{D5: In Fig. 12, the colors of (IND, Drak), (Regroup, Lloyd), (Elka, Drift) look the same to me.}
\response{In the revised manuscript, we have removed those algorithms whose percentages are zero, used labels to distinguish between different algorithms. Please also check the new version in Figure~\ref{fig:lead1}.}

\begin{figure}[h]
	\centering
	\vspace{-1em}
	\includegraphics[height=0.16\textwidth]{graph/pie-time.pdf}
	\includegraphics[height=0.16\textwidth]{graph/pie-time3.pdf}
	\vspace{-1em}
	\caption{{Leaderboard of sequential methods as top 1 \& 3.}}
	\vspace{-2em}
	\label{fig:lead1}
\end{figure}


\setcounter{cN}{0}
\section{Response to Reviewer \#3}
\label{sec:r3}

\comments{W1: Focus on a very narrow domain.}
\response{Clustering is one of the most foundational tasks in data mining and unsupervised learning, which have a wide range of real-world applications, e.g., spatial and GIS analysis, facility location problem, and transport optimizations. %\bao{try to name some applications here.} 
\kmeans has been a very active research topic in both data science and machine learning fields, e.g., the survey on \kmeans \cite{Jain2010} published in 2010  has attracted 7300+ citations. Wu et al. \cite{Wu2008} also identified that \kmeans is one of the top-10 algorithms in data mining (ranked at second place), and this paper has attached 4900+ citations. Moreover, the acceleration for exact \kmeans clustering is also a hot research topic that has attracted much attention, as evidenced by the continuously published papers in top-tier venues such as the most recent one in TPAMI \cite{Xia2020} in July 2020.
In database area, the clustering has also been intensively investigated  in term of efficiency, especially in PVLDB \cite{Bahmani2012,Muller2009,Lulli2016,Wangaclustering}.}

\comments{W2: Not exactly a "Experiments, Analyses \& Benchmarks" paper.}
\response{The guidelines of "Experiments, Analyses \& Benchmarks" paper, which can be accessed from the CFP of PVLDB 2021,\footnote{\url{https://www.vldb.org/pvldb/contributions_vol14.html}} are: 
\textit{
1) fundamentally new insights into the strengths and weaknesses of existing methods or\\
2) new ways to evaluate existing methods.}

We believe that we have met both criteria. Firstly, we have thoroughly compared existing algorithms by reviewing their strengths and weaknesses (see Section~\ref{sec:pre}, \ref{sec:kmeans}, and \ref{sec:seq}), and then conducted experiments over more than ten datasets in Section~\ref{sec:expunik}. Table~\ref{tab:com} has been used to summarize the strengths and weaknesses of the existing algorithms in a more detailed way.
	
\tocheck{Secondly, besides the pruning ratio of distance computation adopted in existing work, we have introduced several new metrics for evaluation, such as data accesses and bound updates which should also be taken into account (see Figures~\ref{fig:seq} to \ref{fig:seq2}). The introduction of our manuscript has also highlighted this as our main motivation (see the green underlines in Section~\ref{sec:moti}). These metrics essentially allow researchers and practitioners to evaluate existing methods (and methods to be proposed in future follow-ups) in a more comprehensive and fine-grained manner.} It is worth mentioning that these metrics have not been used by any existing work, since the pruning ratio of distance computation was thought to be the only evaluation metric apart from the running time. 
	
\tocheck{Thirdly, astute readers may also find that we introduce Section~\ref{sec:auto} titled `Configuration Auto-tuning', which seems to go beyond the basic expectation of an EA\&B paper at first glance. Yes, we did walk extra miles and this is just ``the icing on the cake''. This part plays the role of automatic algorithm selection (a.k.a. recommendation), which is critical to finding the ``most appropriate and best performing'' algorithm, and in turn will be very useful in conducting even a more fair evaluation of different algorithms. For example, by building an algorithm selection model, we are able to identify which problem features are most correlated with the algorithm performance. This provides significant insights into the strengths and weaknesses of an algorithm, and reveals on which type of datasets an algorithm is expected to perform well.} 

%More specifically, this is because we find the algorithm selection is still very hard and current tuning is simply based on hand-crafted decision rules like Figure~\ref{fig:dt}. However, these rules are not applicable in modern systems with various clustering tasks.
%To build preciser and more robust decision rules, we {adopt machine learning models} to automatically select the best method for a given new clustering task in Section~\ref{sec:auto}.
%This is achieved by learning from our evaluation records which contain the performance of all the methods on various datasets. An evaluation on multiple learning models is also conducted in Section~\ref{sec:expauto}. }
%	\bao{I polished this part. But i hope u guys to further polish it, and illustrate how it is going to be useful for evaluation. maybe some details at Sec~6.2 can be moved here.}
}

\comments{W3: Evaluation is not really thorough}
\response{
\tocheck{Unfortunately, since this comment did not provide any detail on which aspect the evaluation is not thorough, we could not provide a specific response to it.} 


\tocheck{We believe that we have conducted a very comprehensive and thorough evaluation, in term of meeting the requirement of an EA\&B paper in the Call For Paper, and comparing with the experimental part of previous relevant studies. 
}

\tocheck{First, please refer to our response to \emph{R3.W2}, which has clearly explained how we have conducted an in-depth and thorough experimental evaluation, in terms of the full coverage of existing methods' pros and cons, and our multiple new evaluation metrics introduced and justified by this work. 
Second, we evaluated more than sixteen approaches over twelve datasets that have a wide coverage of different cardinalities and dimensions, and more importantly highlight which prior studies have used each such dataset (if any). 
Third, our experiments are conducted in three steps smoothly: 1) evaluate existing algorithms; 2) verify our optimization; 3) evaluate our auto-tuning method with various common ML models.}

\tocheck{
Due to space limit, we have to move out some of the results and put into the appendix of our supplementary file, but we think the results in the paper are sufficient to give readers a clear outline of the evaluation. 
Last, we sincerely hope R3 to have another look at Section~\ref{sec:exp}. Should R3 need more details, we refer R3 to the appendix in our supplementary file. For example, in Section~\ref{sec:moreexp} of the appendix, we conducted experiments to study the effect of initialization methods and increasing dimensionality, and then the assignment and refinement speedup in Tables~\ref{tab:assignment} and \ref{tab:refinement}.
Figures~\ref{fig:seqf} to \ref{fig:seq2f} are the full version of Figures~\ref{fig:seq} to \ref{fig:seq2}.
Figures~\ref{fig:s11} to \ref{fig:seq14} show a detailed comparison between sequential methods when setting $k=10$, which mainly enhances Section~\ref{sec:seqexp}.}
%\bao{please better give more specific sections, parts, figures for him to look at in TR.}
}

\comments{Not much effort had been used to use other measurement to compare the algorithm or to generate a proper evaluation datasets. Unik also seems like a research effort on auto-tuning of k-means algorithm rather than a framework to compare and benchmark algorithms.}
\response{This paper provides a comprehensive way to evaluate the \kmeans, e.g., we first review existing algorithms and give a taxonomy of them, then in the experiments we compare existing algorithms in terms of multiple measurements which have never been used, such as data accesses and bound updates (see Figures~\ref{fig:seq} to \ref{fig:seq2}, and the green underlines in Section~\ref{sec:moti}); further, we draw an evaluation summary in Table~\ref{tab:com} to conclude their strengths and weaknesses.
The auto-tuning can be seen as our new insights that can be used to prediction the optimal algorithm for a given clustering task.
For a PVLDB evaluation paper, we understand that new insights and optimizations are also a core part, as they are essential to solve the urgent problem we face during the evaluation, just like many PVLDB evaluation papers did \cite{Yang2015a,Abeywickrama2016}. We also suggest that the reviewer refers to our response to comment 2 of meta-review in Section~\ref{sec:meta} for more information.}

\vspace{-1em}
\section{Other Improvements}
\label{sec:newmethod}
Here, we also report other improvement we did to further enhance the quality of this work, although it is not required by the reviewers or meta-reviewer.
%\newcontent{We add a new work here}
%\textbf{\textcolor{Brown}{\underline{\textbf{}}.~}}
\subsubsection{A new method is added and evaluated}
As shown in Figure~\ref{fig:timeline}, we present the research timeline of fast \kmeans, and try to keep track of every important algorithm and make the timeline complete. We will also keep updating this if we find a new algorithm in the future.
During our revision, we noticed that a highly related paper was just accepted by the TPAMI journal (one of the top-tier journals on machine learning) on \textbf{13 July 2020}, called ``\textit{A Fast Adaptive k-means with No Bounds'}' \cite{Xia2020}.\\

\noindent\fbox{
	\parbox{0.46\textwidth}{
\textit{Xia S, Peng D, Meng D, Zhang C, Wang G, Giem E, Wei W, Chen Z. A Fast Adaptive k-means with No Bounds. IEEE Transactions on Pattern Analysis and Machine Intelligence. 2020 Jul 13. \url{https://ieeexplore.ieee.org/document/9139397}}}}\\

To further complete this experimental evaluation, we believe it is our obligation to include it, although it was published online (early access) just two days before we got revision notification of our PVLDB submission on \textbf{15 July 2020}.
In particular, we implemented it in our framework \uni and added a short description in Section~\ref{sec:pami20} as it belongs the group of methods that use less bounds. 
We also updated the timeline in Figure~\ref{fig:timeline}, and Algorithm~\ref{alg:kmeans}.

We named this new method as ``\texttt{Pami20}'' and updated the corresponding results in the experiments.
Please check the Figures~\ref{fig:seq} to \ref{fig:seq2}. We found this method can save much space without using bound for every data point, and can still achieve considerable performance, which is consistent with the claim of their paper. 
However, it has a low probability being one of the top-3 fastest methods and the probability of being the fastest is almost zero, as shown in Figure~\ref{fig:lead}.
%Hence, the rule that exchanging space for efficiency still applies here.

This method is not the fastest among all algorithms in our experiments because their pruning only depends on the centroid distance, which is not enough to be effective like other bounds that exchange space for high performance. Another reason is that most datasets tested in the paper \cite{Xia2020} are relatively small ($n\le141,690$) and quite different from most existing work.
Moreover, the indexing methods \cite{Moore2000} \cite{Kanungo2002} are not compared; only six methods were compared, while we have 15.
In their experiments, the results also indicate that \texttt{Pami20} can only have a 71\% probability to be the fastest method among the six methods (check their Table 4).
Based on the fact that \texttt{Pami20} has a low probability of being the fastest one when no advanced bounds are used, we still choose the original five representative sequential methods to conduct further experiments in Section~\ref{sec:expauto}.
%We also fixed several small typos to improve the overall presentation. We will keep polishing it.

